ModelTalk: A Framework for Developing Domain Specific Executable Models

Developing and maintaining complex, large-scale, product line of highly customized software systems is difficult and costly. Part of the difficulty is due to the need to communicate business knowledge between domain experts and application programmers. Domain specific model driven development (MDD) addresses this difficulty by providing domain experts and developers with domain specific abstractions for communicating designs. Most MDD implementations take a generative approach. In contrast, we adopt an interpretive approach to domain specific model driven development. We present a framework, named ModelTalk, that integrates MDD, dependency injection and meta-modeling to form an interpretive, domain specific modeling framework. The framework is complemented by tool support that provides developers with the same advanced level of usability for modeling as they are accustomed to in programming environments. ModelTalk is used in a commercial setting for developing a product line of Telco grade business support systems (BSS).

==> abstract.txt <==
ModelTalk: A Framework for Developing Domain Specific Executable Models

Atzmon Hen-Tov, Pontis, Glil Yam 46905, Israel {atzmon@pontis.com}
David H. Lorenz, The Open University of Israel, 108 Ravutski St., Raanana 43107, Israel {lorenz@openu.ac.il}
Lior Schachter, Pontis, Glil Yam 46905, Israel {liors@pontis.com}

Abstract:

Developing and maintaining complex, large-scale, product line of highly
customized software systems is difficult and costly.  Part of the
difficulty is due to the need to communicate business knowledge between
domain experts and application programmers.  Domain specific model driven
development (MDD) addresses this difficulty by providing domain experts
and developers with domain specific abstractions for communicating
designs.  Most MDD implementations take a generative approach.
In contrast, we adopt an interpretive approach to domain specific
model driven development.  We present a framework, named ModelTalk,
that integrates MDD, dependency injection and meta-modeling to form
an interpretive, domain specific modeling framework.  The framework
is complemented by tool support that provides developers with the same
advanced level of usability for modeling as they are accustomed to in
programming environments.  ModelTalk is used in a commercial setting
for developing a product line of Telco grade business support systems
(BSS).

\category{D2.6}{Programming Environments}{Programmer workbench}
\category{D3.2}{Language Classifications}{Extensible languages, Object-oriented languages}

\terms
Design, Languages

\keywords
Model driven development; Dependency injection; Meta-modeling; Executable model; Domain specific languages 

